Exact solution of generalized gauge-invariant Ising chains with multi-spin interactions

In this work, exact solutions are obtained for a class of generalized gauge-invariant $n$-chain Ising models ($n=1,2,3,4$) with arbitrary multi-spin interactions that are invariant under the local $\mathbb{Z}_2$ gauge group. On a strip lattice of finite length $L$ and width $n$ with periodic or free boundary conditions, an explicit expression for the partition function is derived using the transfer-matrix method. Two successive transformations are developed: elimination of gauge redundancy and reduction of the original model to an effective $n$-chain Ising model with all possible interactions between neighboring vertical layers. On the basis of the spectral decomposition of the $2^n\times 2^n$ transfer matrix, general formulas are obtained for gauge-invariant correlation functions and Wilson loops of arbitrary width. For $n \le 3$, explicit expressions are derived in terms of eigenvalues and eigenvectors. A detailed analysis of the behavior of the Wilson loop is performed, which allows us to identify regimes exhibiting area-law (confinement-like) and perimeter-law (deconfinement-like) dependence. For specific Hamiltonians, the string tension is computed and the corresponding phase diagrams are constructed. The results generalize and substantially extend the classical works on the gauge-invariant Ising model.

==> Parts/Conslusion.tex <==
	In this work we have obtained exact solutions for the class of generalized gauge-invariant $n$-chain Ising models ($n=1,2,3,4$) with arbitrary multi-spin interactions invariant under the local $\mathbb{Z}_2$ group. Using two successive transformations --- elimination of gauge redundancy and reduction to an effective $n$-chain Ising model --- the problem is reduced to the spectral analysis of a $2^n\times 2^n$ transfer matrix. Explicit expressions are derived for the partition function, gauge-invariant correlation functions, and Wilson loops of arbitrary width. For $n\le 3$ the formulas are given in closed form in terms of eigenvalues and eigenvectors. A detailed analysis of the Wilson-loop behavior makes it possible to identify confinement-like (area-law) and deconfinement-like (perimeter-law) regimes and to compute the string tension. The results significantly extend the classical studies of the gauge-invariant Ising model and open the way to further analytical and numerical investigations of higher-dimensional generalizations and phase diagrams.


==> Parts/Literature.tex <==
\newpage
\begin{thebibliography}{bibliography}
				
    \bibitem{Ising}
    \newblock Ising E., Beitrag zur Theorie des 
    Ferromagnetismus, Zeitschrift fűr Physik, 31 (1925), 253-258.
    DOI:10.1007/bf02980577
    
    \bibitem{Onsager}
    \newblock Onsager L., Crystal 
    statistics. I. A two-dimensional model with an order–disorder transition, Physical 
    Review, 65(3-4) (1944), 117-149. DOI: 10.1103/Phys-Rev.65.117
    
    \bibitem{Kramers1}
    \newblock Kramers H. A., Wannier G. H. Statistics 
    of the two-dimensional ferromagnet. Part I //Physical Review. – 1941. – Т. 60. – №. 3. – С. 252.
    DOI:10.1103/physrev.60.252
    
    \bibitem{Kramers2}
    \newblock Kramers H. A., Wannier G. H. Statistics of the two-dimensional 
    ferromagnet. Part II //Physical Review. – 1941. – Т. 60. – №. 3. – С. 263.
    DOI:10.1103/physrev.60.263
    
    \bibitem{Kogut}
    \newblock Kogut, J. B. (1979). An introduction to lattice gauge theory and spin systems. Reviews of Modern Physics, 51(4), 659. 
    DOI:10.1103/RevModPhys.51.659

    \bibitem{Marra_Miracle-Sole}
    \newblock Marra, R., \& Miracle-Sole, S. (1979). On the statistical mechanics of the gauge invariant Ising model. Communications in Mathematical Physics, 67, 233-240.
    DOI:10.1007/bf01238846

    
    \bibitem{Nauenberg}
    \newblock Nauenberg, M. (1981). Correlation and specific heat of U(1) and SU(2) lattice gauge models. Phys. Scr., 23(5, pt.2), 981–982.
    DOI:10.1088/0031-8949/23/5b/013

    \bibitem{Peskin}
    \newblock Peskin, M.E. (1995). An Introduction To Quantum Field Theory (1st ed.). CRC Press.
    DOI:10.1201/9780429503559

    \bibitem{Balian}
    \newblock Balian, R., J. M. Drouffe, and Claude Itzykson. "Gauge fields on a lattice. II. Gauge-invariant Ising model." Physical Review D 11.8 (1975): 2098.

    
    \bibitem{Yokota}
    \newblock Yokota, T. (1989). Pair correlations for double-chain and triple-chain Ising models with competing interactions. Physical Review B, 39(16), 12312–12315. DOI:10.1103/physrevb.39.12312
    
    \bibitem{Kalok}
    \newblock Kalok, L., and L. C. De Menezes. "Competing interactions in double-chains: Ising and spherical models." Zeitschrift für Physik B Condensed Matter 20.2 (1975): 223-229.
    DOI:10.1007/bf01315695 
    
    \bibitem{Baxter1}
    \newblock Baxter, R.J. Exactly Solved Models in Statistical Mechanics; Academic Press: San Diego, California, USA, 2016; ISBN 0-12-083180-5.

    %!!!!!!!!!!!!!!!!!!!
    \bibitem{Baxter2}
    \newblock Baxter, R. J. (1986). The Yang-Baxter equations and the Zamolodchikov model. Physica D: Nonlinear Phenomena, 18(1-3), 321-347. DOI:10.1016/0167-2789(86)90195-8
  
    
    \bibitem{Malyshev_VA_Minlos_RA}
    \newblock Malyshev, V. A., and Minlos, R. A. (2012). Gibbs random fields: cluster expansions (Vol. 44). Springer Science and Business Media.
    
    
    \bibitem{Khrapov_PV}
    \newblock Khrapov, P. V. (1984). Cluster expansion and spectrum of the transfer matrix of the two-dimensional ising model with strong external field. Theoretical and Mathematical Physics, 60(1), 734–735. 
    DOI:10.1007/bf01018259 
    
    
    \bibitem{Khrapov_PV_Nikishina_VA}
    \newblock Khrapov, Pavel, and Veronika Nikishina. Exact solution Ising-like $2\times 2\times\infty $ models with multispin interactions. arXiv preprint arXiv:2205.15640 (2022). DOI: 10.48550/arXiv.2205.15640
    
            
    

    \bibitem{Volkov_Khrapov}
    \newblock Khrapov, P., \& Volkov, N. (2024). Exact solution of generalized triple Ising chains with multi-spin interactions. arXiv preprint arXiv:2406.10683.
    DOI:10.48550/arXiv.2406.10683

    \bibitem{Cardano}
    \newblock Cardano G., Witmer T. R., Ore O. The rules of algebra: Ars Magna. – Courier Corporation, 2007. – Т. 685.

    \bibitem{Wegner}
    \newblock Franz J. Wegner, Duality in Generalized Ising Models and Phase Transitions without Local Order Parameters, Journal of Mathematical Physics 12 (1971), 2259–2272. DOI: 10.1063/1.1665530.

    \bibitem{Wilson}
    \newblock Kenneth G. Wilson, Confinement of quarks, Physical Review D 10 (1974), 2445–2459. DOI: 10.1103/PhysRevD.10.2445.

    \bibitem{Elitzur}
    \newblock Shmuel Elitzur, Impossibility of spontaneously breaking local symmetries, Physical Review D 12 (1975), 3978–3982. DOI: 10.1103/PhysRevD.12.3978.

    \bibitem{Savit}
    \newblock Robert Savit, Duality in field theory and statistical systems, Reviews of Modern Physics 52 (1980), 453–487. DOI: 10.1103/RevModPhys.52.453.

    \bibitem{Turban}
    \newblock  Loïc Turban, One-dimensional Ising model with multispin interactions, Journal of Physics A:Mathematical and Theoretical 49 (2016), 355002. DOI: 10.1088/1751-8113/49/35/355002.
    
\end{thebibliography}
